Stability estimates for adaptive focused time-frequency transforms

This contribution is a follow-up of a recent paper by the authors on adaptive, non-linear time-frequency transforms, focusing on the STFT based transforms. The adaptivity is provided by a focus function, that depends on the analyzed function or signal, and that adapts dynamically the time-frequency resolution of the analysis. Sticking to the continuous case setting, this work provides new stability results for the transform (stability with respect with the focus function). It also investigates in some details focus functions based upon regularized R{\'e}nyi entropies and show corresponding continuity results.

==> focus_function_entropy.tex <==
\section{Focus function through entropy measure}

\subsection{Renyi based focus function}

In the first paper we gave illustration with entropy based focus functions but it was in discrete case.

\subsection{Estimate of the focus function}

==> frequency_focused_transform.tex <==
\section{Frequency-focused transform}
\subsection{Definition}

For the frequency focused transform we took a completely different approach...

The assumptions are:
\begin{enumerate}[i.]
\item 
$\psi\in H^2(\R)$ is an analytic wavelet function, therefore satisfying the admissibility condition~\eqref{fo:CWT.admissibility.H2}, and such that the quantity below (called frequency localization of $\psi$) is well-defined.
\label{FFTFT.assumption.psi}
\begin{equation}
\label{eq_wavelet_freq_loc}
\xi_0 := \frac{1}{\|\psi\|^2}\int_{\R_+} \xi |\hat\psi(\xi)|^2\,d\xi\ .    
\end{equation}
In addition, we assume that $|\hat\psi|^2$ is differentiable, and make the following technical assumptions:
\begin{itemize}
\item
$\hat\psi(\xi_0)\ne 0$
\item 
There exists $A_\psi>0$ such that for all $\xi\in\R_+$, 
\begin{equation}
\label{eq_hypothesis_psi}
\left(|\hat\psi|^2\right)'(\xi) \le \frac{A_\psi}{|\xi-\xi_0|}\ .
\end{equation}
\end{itemize}
%For technical reasons, we will make the following hypotheses \bruno{(toujours d'actualité ?)}\pierre{Oui normalement}
%\begin{equation}\label{eq_hypothesis_psi}
%\exists A_\psi,B_\psi >0 \text{ such that } \ \forall y\in\R, \  |y||\hat{\psi}(\xi_0+y)|\leqslant A_\psi \ \text{ and } \ \hat{\psi}'\in L^\infty
%\end{equation}
\item
$\gamma$ denotes a positive, strictly increasing $C^1$ diffeomorphism that maps $\R$ onto $\R_+^*$. 
\item
To every $f\in L^2(\R)$ is associated a focus function $\sigma^\nu_f$ of $f\in L^2(\R)$, assumed to be  continuous, larger than 1 and such that $\sigma_f^\nu -1$ goes to 0 at $\pm\infty$:
\begin{equation}
	\forall f\in L^2(\R), \quad \sigma^\nu_f \in C_{0}^+(\R) + 1\ .
\end{equation}
\end{enumerate}

With such assumptions we define the frequency-focused atoms by their Fourier transform for $t,u,\xi\in\R$
\begin{equation}
\widehat{\psi_{t,u,\sigma}}(\xi)=\frac{1}{\sqrt{\gamma(u)}}\,\hat\psi\left(\beta_u(\xi)\right)e^{-2i\pi\xi t}\ .
\end{equation}
And the frequency-focused operator for $f\in L^2(\R)$ and $t,u\in\R$,
\begin{equation}
   M^\nu f(t,u) := \langle f , \psi_{t,u,\sigma_f^\nu}\rangle_{L^2}.
\end{equation}

\subsection{Norm control}


\begin{theorem}[Warion, Torrésani, 2024]\label{theorem_norm_control_frequency_focus}
Let $\psi$ satisfying assumptions~\ref{FFTFT.assumption.psi}. in Section~{\ref{ssec:def.FFTFT}}.
	Let $f\in H^2(\R)$,
 %$\psi$ satisfying hypothesis~\eqref{eq_hypothesis_psi}
 and let $\sigma^\nu_f\in C_0^+(\R)+1$ denote the associated frequency-focus function.
 %, lets $0<a<b<+\infty$ such that
    Then we have
	\begin{equation}
		d_\psi\|f\|_{L^2(\R)}^2 \leqslant \|M^\nu f \|_{L^2(\R^2,d\mu)}^2 \leqslant C_{\sigma_f^\nu}\|f\|_{L^2(\R)}^2\ ,
	\end{equation}
	where $d_\psi>0$ depends only on the wavelet $\psi$, and $C_{\sigma_f^\nu}$ is given by
	\begin{equation}
		C_{\sigma_f^\nu} := c_\psi + A_\psi\ \int_{\R_+}\left(\sigma_f^\nu(\gamma^{-1}(y))-1\right)\frac{dy}{y} <+\infty,
	\end{equation}
%	\begin{equation}
%		c_{a,b}^2 := \frac{|\hat{\psi}(\xi_0)|^2}{2}\ln\left(\frac{b}{a}\right).
%	\end{equation}
\end{theorem}


